Prediction of Rare Channel Conditions using Bayesian Statistics and Extreme Value Theory

Estimating the probability of rare channel conditions is a central challenge in ultra-reliable wireless communication, where random events, such as deep fades, can cause sudden variations in the channel quality. This paper proposes a sample-efficient framework for predicting the statistics of such events by utilizing spatial dependency between channel measurements acquired from various locations. The proposed framework combines radio maps with non-parametric models and extreme value theory (EVT) to estimate rare-event channel statistics under a Bayesian formulation. The framework can be applied to a wide range of problems in wireless communication and is exemplified by rate selection in ultra-reliable communications. Notably, besides simulated data, the proposed framework is also validated with experimental measurements. The results in both cases show that the Bayesian formulation provides significantly better results in terms of throughput compared to baselines that do not leverage measurements from surrounding locations. It is also observed that the models based on EVT are generally more accurate in predicting rare-event statistics than non-parametric models, especially when only a limited number of channel samples are available. Overall, the proposed methods can significantly reduce the number of measurements required to predict rare channel conditions and guarantee reliability.

==> sections/estimation_bias.tex <==
We conclude the section by discussing the behavior of the coverage guarantee, i.e., $P(X_{\epsilon} \in I(\mathcal{D}))$, as the number of observations $n$ at the new user location $\mbf{s}_0$ increases. In particular, the impact of a potential model bias.

Assume a one-sided confidence interval $I_n(\mathcal{D}) = [I_{\min,n}
(\mathcal{D}), \infty)$ (slightly changing the previous notation to emphasize the dependence on $n$). As $n$ increases, it is reasonable to assume that the confidence interval converges. Formally, we assume that $I_{\min,n}(\mathcal{D})$ converges in probability, denoted $I_{\min,n}(\mathcal{D}) \overset{p}{\to} I_{\min}$ for $n \to \infty$ where $I_{\min} > 0$ is the limit for the lower bound. We can always write $I_{\min} = X_{\epsilon} + b$ where $b$ is the \textit{bias} with respect to the true $\epsilon$-quantile $X_{\epsilon}$. A bias can occur if the model used to infer the confidence interval differs from the probability distribution of $X$ and we say that the confidence interval is \textit{inconsistent}, which will be the case in most practical  scenarios. In particular, while the \gls{gpd} models used in Sec. \ref{subsec:evt_bayesian} and \ref{subsubsec:evt_baseline} are asymptotically correct, there will be some bias for any constant choice of $\epsilon$. This leads to the next theorem: \TK{Agree with the terminoligy Christophe?}
\begin{theorem} \label{thm:convergence_onesided}
    Assume an inconsistent one-sided confidence interval $I_n(\mathcal{D})$ whose lower bound converges in probability to some constant $I_{\min}$. Letting $b = I_{\min} - X_{\epsilon}$, it follows that:
    \begin{align}
        b > 0 &\Rightarrow P(X_{\epsilon} \in I_n(\mathcal{D})) \overset{p}{\to} 0 \ \ \text{for} \ \ n \to \infty,\label{eq:statement_positive_bias} \\
        b < 0 &\Rightarrow P(X_{\epsilon} \in I_n(\mathcal{D})) \overset{p}{\to} 1 \ \ \text{for} \ \ n \to \infty. \label{eq:statement_negative_bias}
    \end{align}
\end{theorem}
\begin{IEEEproof}
    See Appendix \ref{subsec:proof_thm2}.
  \end{IEEEproof}
\AK{Maybe I don't understand the theorem, but the way I read it is this: an inconsistent estimator of the quantile that converges to a quantile greater than the true quantile will not converge to a quantile less than the true quantile. Also, what do you mean when you say that $P(X_{\epsilon} \in I_n(\mathcal{D}))$ converges in probability? Is $P(X_{\epsilon} \in I_n(\mathcal{D}))$ a random variable? Or you mean the event $\mathbbm{1}[X_{\epsilon} \in I_n(\mathcal{D})]$?}
Theorem \ref{thm:convergence_onesided} states that the coverage guarantee converges to either $0$ or $1$ depending on a positive or negative bias, respectively. Intuitively, this is because, as the lower bound $I_{\min,n}(\mathcal{D})$ converges to the limit $I_{\min}$, any non-zero bias will cause the estimate to either under or overestimate the quantile $X_{\epsilon}$. A corollary to Theorem \ref{thm:convergence_onesided} is that, for a two-sided confidence interval $I_{n}(\mathcal{D}) = [I_{\min,n}(\mathcal{D}),I_{\max,n}(\mathcal{D})]$, if $I_{n}(\mathcal{D})$ converges in probability to a point $I \in \mR$, then any non-zero bias $b = I - X_{\epsilon} \neq 0$ will cause $P(X_{\epsilon} \in I_n(\mathcal{D})) \overset{p}{\to} 0$ (the proof is similar to the one in Appendix \ref{subsec:proof_thm2} and omitted here). 

There are some key takeaways from this discussion. First, providing a correct coverage guarantee is generally difficult in the high-sample domain since any model bias will tend to dominate as the number of observations grows. Secondly, non-parametric methods can avoid the bias problem by not relying on a model, which is an argument for using non-parametric models in the high-sample domain.  Finally, although even a small bias $b \approx 0$ may cause the coverage guarantee to be violated, the estimated confidence interval can still be accurate. For example, in the one-sided case, the estimation error fulfills $|X_{\epsilon} - I_{\min,n}| \overset{p}{\to} b \approx 0$ given the previous assumptions. We will illustrate these observations numerically in Sec. \ref{sec:rate_selection}.

